Adaptive Methods for Multiobjective Unit Commitment

This work considers a multiobjective version of the unit commitment problem that deals with finding the optimal generation schedule of a firm, over a period of time and a given electrical network. With growing importance of environmental impact, some objectives of interest include CO2 emission levels and renewable energy penetration, in addition to the standard generation costs. Some typical constraints include limits on generation levels and up/down times on generation units. This further entails solving a multiobjective mixed integer optimization problem. The related literature has predominantly focused on heuristics (like Genetic Algorithms) for solving larger problem instances. Our major intent in this work is to propose scalable versions of mathematical optimization based approaches that help in speeding up the process of estimating the underlying Pareto frontier. Our contributions are computational and rest on two key embodiments. First, we use the notion of both epsilon constraints and adaptive weights to solve a sequence of single objective optimization problems. Second, to ease the computational burden, we propose a Mccormick-type relaxation for quadratic type constraints that arise due to the resulting formulation types. We test the proposed computational framework on real network data from [1,50] and compare the same with standard solvers like Gurobi. Results show a significant reduction in complexity (computational time) when deploying the proposed framework.

==> pic2e.tex <==
%%
%% This is file `pict2e.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pict2e.dtx  (with options: `package')
%%
%% Copyright (C) 2003, 2004, 2008
%% Rolf Niepraschk, Rolf.Niepraschk@ptb.de
%% Hubert Gaesslein, HubertJG@open.mind.de
%% Josef Tkadlec, j.tkadlec@email.cz
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "author-maintained".
%%
%% This work consists of all files listed in `manifest.txt'.
%%
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{pict2e}
  [2008/07/22 v0.2w Improved picture commands (HjG,RN,JT)]
\edef\Gin@codes{%
 \catcode`\noexpand\^^A\the\catcode`\^^A\relax
 \catcode`\noexpand\"\the\catcode`\"\relax
 \catcode`\noexpand\!\the\catcode`\!\relax
 \catcode`\noexpand\:\the\catcode`\:\relax}
\catcode`\^^A=\catcode`\%
\@makeother\"%
\@makeother\!%
\@makeother\:%
\newcommand*\pIIe@mode{-1}
\newcommand*\pIIe@code[1]{}
\providecommand*\Gin@driver{}
\newcommand*\pIIe@tempa{}
\newcommand*\pIIe@tempb{}
\newcommand*\pIIe@tempc{}
\DeclareOption{dvips}{\def\Gin@driver{dvips.def}}
\DeclareOption{xdvi}{\ExecuteOptions{dvips}}
\DeclareOption{dvipdf}{\def\Gin@driver{dvipdf.def}}
\DeclareOption{dvipdfm}{\def\Gin@driver{dvipdfm.def}}
\DeclareOption{pdftex}{\def\Gin@driver{pdftex.def}}
\DeclareOption{dvipsone}{\def\Gin@driver{dvipsone.def}}
\DeclareOption{dviwindo}{\ExecuteOptions{dvipsone}}
\DeclareOption{oztex}{\ExecuteOptions{dvips}}
\DeclareOption{textures}{\def\Gin@driver{textures.def}}
\DeclareOption{pctexps}{\def\Gin@driver{pctexps.def}}
\DeclareOption{pctex32}{\def\Gin@driver{pctex32.def}}
\DeclareOption{vtex}{\def\Gin@driver{vtex.def}}
\DeclareOption{original}{\def\pIIe@mode{0}}
\DeclareOption{ltxarrows}{\AtEndOfPackage{%
  \let\pIIe@vector=\pIIe@vector@ltx
  \def\pIIe@FAL{1.52}%
  \def\pIIe@FAW{3.2}%
  \def\pIIe@CAW{1.5pt}%
  \def\pIIe@FAI{0.25}%
  }}
\DeclareOption{pstarrows}{\AtEndOfPackage{%
  \let\pIIe@vector=\pIIe@vector@pst
  \iffalse
    \def\pIIe@FAL{1.4}%
    \def\pIIe@FAW{2}%
    \def\pIIe@CAW{1.5pt}%
    \def\pIIe@FAI{0.4}%
  \else % These are the ltxarrows values, which looks better. (RN)
    \def\pIIe@FAL{1.52}%
    \def\pIIe@FAW{3.2}%
    \def\pIIe@CAW{1.5pt}%
    \def\pIIe@FAI{0.25}%
  \fi
  }}
\newcommand*\pIIe@debug@comment{}
\DeclareOption{debug}{%
  \def\pIIe@debug@comment{^^J^^J\@percentchar\space >>> pict2e <<<^^J}%
  \begingroup
    \@ifundefined{pdfcompresslevel}{}{\global\pdfcompresslevel\z@}%
  \endgroup}
\DeclareOption{hide}{\AtEndOfPackage{%
  \let\pIIe@code\@gobble
}}
\DeclareOption*{\ExecuteOptions{original}}
\ExecuteOptions{ltxarrows}
\InputIfFileExists{pict2e.cfg}{}{}
\ProcessOptions\relax
\ifnum\pIIe@mode=\z@
  \PackageInfo{pict2e}{Package option `original' requested}
\else
  \if!\Gin@driver!
    \PackageError{pict2e}
      {No driver specified at all}
      {You should make a default driver option in a file\MessageBreak
       pict2e.cfg\MessageBreak eg: \protect\ExecuteOptions{dvips}}%
  \else
    \PackageInfo{pict2e}{Driver file: \Gin@driver}
    \@ifundefined{ver@\Gin@driver}{\input{\Gin@driver}}{}
    \PackageInfo{pict2e}{Driver file for pict2e: p2e-\Gin@driver}
    \InputIfFileExists{p2e-\Gin@driver}{}{%
      \PackageError{pict2e}%
        {Driver file ``p2e-\Gin@driver'' not found}%
        {Q: Is the file properly installed? A: No!}}
  \fi
\fi
\ifnum\pIIe@mode>\z@
  \ifnum\pIIe@mode<\thr@@
    \RequirePackage{trig}
    \let\pIIe@oldline\line
    \let\pIIe@old@sline\@sline
    \let\pIIe@oldvector\vector
    \let\pIIe@old@circle\@circle
    \let\pIIe@old@dot\@dot
    \let\pIIe@old@bezier\@bezier
    \AtBeginDocument{%
      \@ifundefined{@cbezier}{%
        \def\pIIe@old@cbezier[#1](#2,#3)(#4,#5)(#6,#7)(#8,#9){}%
        }{\let\pIIe@old@cbezier\@cbezier}}
    \let\pIIe@oldoval\oval
    \let\pIIe@old@oval\@oval
    \newcommand*\OriginalPictureCmds{%
      \let\@sline\pIIe@old@sline
      \let\line\pIIe@oldline
      \let\vector\pIIe@oldvector
      \let\@circle\pIIe@old@circle
      \let\@dot\pIIe@old@dot
      \let\@bezier\pIIe@old@bezier
      \let\@cbezier\pIIe@old@cbezier
      \renewcommand*\oval[1][]{\pIIe@oldoval}%
      \let\@oval\pIIe@old@oval
    }
  \else
    \PackageError{pict2e}
      {Unsupported mode (\pIIe@mode) specified}
      {The driver you specified requested a mode\MessageBreak
       not supported by this version of this package}
  \fi
\else
  \ifnum\pIIe@mode<\z@
    \PackageError{pict2e}
      {No suitable driver specified}
      {You should make a default driver option in a file\MessageBreak
       pict2e.cfg\MessageBreak eg: \protect\ExecuteOptions{dvips}}
  \fi
\fi
\ifnum\pIIe@mode>\z@
  \ifcase\pIIe@mode\relax
  \or
    \newcommand*\pIIe@moveto@op{moveto}
    \newcommand*\pIIe@lineto@op{lineto}
    \newcommand*\pIIe@setlinewidth@op{setlinewidth}
    \newcommand*\pIIe@stroke@op{stroke}
    \newcommand*\pIIe@fill@op{fill}
    \newcommand*\pIIe@curveto@op{curveto}
    \newcommand*\pIIe@concat@op{concat}
    \newcommand*\pIIe@closepath@op{closepath}
  \or
    \newcommand*\pIIe@moveto@op{m}
    \newcommand*\pIIe@lineto@op{l}
    \newcommand*\pIIe@setlinewidth@op{w}
    \newcommand*\pIIe@stroke@op{S}
    \newcommand*\pIIe@fill@op{f}
    \newcommand*\pIIe@curveto@op{c}
    \newcommand*\pIIe@concat@op{cm}
    \newcommand*\pIIe@closepath@op{h}
  \fi
  \@ifdefinable\pIIe@GRAPH{\newtoks\pIIe@GRAPH}
  \newcommand*\pIIe@addtoGraph[1]{%
    \begingroup
      \edef\x{\the\pIIe@GRAPH\space#1}%
      \global\pIIe@GRAPH\expandafter{\x}%
    \endgroup}
  \newcommand*\pIIe@fillGraph{\begingroup \@tempswatrue\pIIe@drawGraph}
  \newcommand*\pIIe@strokeGraph{\begingroup \@tempswafalse\pIIe@drawGraph}
  \newcommand*\pIIe@drawGraph{%
      \edef\x{\pIIe@debug@comment\space
              \pIIe@scale@PTtoBP}%
      \if@tempswa
        \edef\y{\pIIe@fill@op}%
      \else
        \edef\x{\x\space\strip@pt\@wholewidth
          \space\pIIe@setlinewidth@op}%
        \edef\y{\pIIe@stroke@op}%
      \fi
      \expandafter\pIIe@code\expandafter{%
        \expandafter\x\the\pIIe@GRAPH\space\y}%
      \global\pIIe@GRAPH{}\xdef\pIIe@CPx{}\xdef\pIIe@CPy{}%
    \endgroup}
  \newcommand*\pIIe@CPx{} \newcommand*\pIIe@CPy{}
  \newcommand*\pIIe@add@CP[2]{%
    \begingroup
      \@tempdima#1\xdef\pIIe@CPx{\the\@tempdima}%
      \@tempdimb#2\xdef\pIIe@CPy{\the\@tempdimb}%
      \pIIe@addtoGraph{\strip@pt\@tempdima\space\strip@pt\@tempdimb}%
    \endgroup}
  \newcommand*\pIIe@add@nums[2]{%
    \begingroup
      \@tempdima#1\relax
      \@tempdimb#2\relax
      \pIIe@addtoGraph{\strip@pt\@tempdima\space\strip@pt\@tempdimb}%
    \endgroup}
  \newcommand*\pIIe@add@num[1]{%
    \begingroup
      \@tempdima#1\relax
      \pIIe@addtoGraph{\strip@pt\@tempdima}%
    \endgroup}
  \newcommand*\pIIe@PTtoBP{0.99626401 }
  \ifcase\pIIe@mode\relax
  \or
    \newcommand*\pIIe@concat[6]{%
      \begingroup
        \pIIe@addtoGraph{[}%
        \@tempdima#1\relax \@tempdimb#2\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#3\relax \@tempdimb#4\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#5\relax \@tempdimb#6\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \pIIe@addtoGraph{] \pIIe@concat@op}%
      \endgroup}
    \newcommand*\pIIe@translate[2]{\pIIe@add@nums{#1}{#2}\pIIe@addtoGraph{translate}}
    \newcommand*\pIIe@rotate[1]{\pIIe@add@num{#1}\pIIe@addtoGraph{rotate}}
    \newcommand*\pIIe@scale[2]{\pIIe@add@nums{#1}{#2}\pIIe@addtoGraph{scale}}
    \newcommand*\pIIe@scale@PTtoBP{\pIIe@PTtoBP \pIIe@PTtoBP scale}
  \or
    \newcommand*\pIIe@concat[6]{%
      \begingroup
        \@tempdima#1\relax \@tempdimb#2\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#3\relax \@tempdimb#4\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#5\relax \@tempdimb#6\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \pIIe@addtoGraph\pIIe@concat@op
      \endgroup}
    \newcommand*\pIIe@translate[2]{\pIIe@concat\p@\z@\z@\p@{#1}{#2}}
    \newcommand*\pIIe@rotate[1]{%
      \begingroup
        \@tempdima#1\relax
        \edef\pIIe@tempa{\strip@pt\@tempdima}%
        \CalculateSin\pIIe@tempa
        \CalculateCos\pIIe@tempa
        \edef\pIIe@tempb{\UseSin\pIIe@tempa}%
        \edef\pIIe@tempc{\UseCos\pIIe@tempa}%
        \pIIe@concat{\pIIe@tempc\p@}{\pIIe@tempb\p@}%
          {-\pIIe@tempb\p@}{\pIIe@tempc\p@}\z@\z@
      \endgroup}
    \newcommand*\pIIe@scale[2]{\pIIe@concat{#1}\z@\z@{#2}\z@\z@}
    \newcommand*\pIIe@scale@PTtoBP{\pIIe@PTtoBP 0 0 \pIIe@PTtoBP 0 0 \pIIe@concat@op}
  \fi
  \newcommand*\pIIe@moveto[2]{%
    \pIIe@add@CP{#1}{#2}\pIIe@addtoGraph\pIIe@moveto@op}
  \newcommand*\pIIe@lineto[2]{%
    \pIIe@add@CP{#1}{#2}\pIIe@addtoGraph\pIIe@lineto@op}
  \ifcase\pIIe@mode\relax
  \or
    \newcommand*\pIIe@rcurveto[6]{%
      \begingroup
        \@tempdima#1\relax \@tempdimb#2\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#3\relax \@tempdimb#4\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#5\relax \@tempdimb#6\relax
        \pIIe@add@CP\@tempdima\@tempdimb
        \pIIe@addtoGraph{rcurveto}%
      \endgroup}
  \or
    \newcommand*\pIIe@rcurveto[6]{%
      \begingroup
        \@tempdima#1\advance\@tempdima\pIIe@CPx\relax
        \@tempdimb#2\advance\@tempdimb\pIIe@CPy\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#3\advance\@tempdima\pIIe@CPx\relax
        \@tempdimb#4\advance\@tempdimb\pIIe@CPy\relax
        \pIIe@add@nums\@tempdima\@tempdimb
        \@tempdima#5\advance\@tempdima\pIIe@CPx\relax
        \@tempdimb#6\advance\@tempdimb\pIIe@CPy\relax
        \pIIe@add@CP\@tempdima\@tempdimb
        \pIIe@addtoGraph\pIIe@curveto@op
      \endgroup}
  \fi
  \newcommand*\pIIe@curveto[6]{%
    \begingroup
      \@tempdima#1\relax \@tempdimb#2\relax
      \pIIe@add@nums\@tempdima\@tempdimb
      \@tempdima#3\relax \@tempdimb#4\relax
      \pIIe@add@nums\@tempdima\@tempdimb
      \@tempdima#5\relax \@tempdimb#6\relax
      \pIIe@add@CP\@tempdima\@tempdimb
      \pIIe@addtoGraph\pIIe@curveto@op
    \endgroup}
  \newcommand*\pIIe@closepath{\pIIe@addtoGraph\pIIe@closepath@op}
  \newcommand*\pIIe@pyth[3]{%
    \begingroup
      \@tempdima=#1\relax
      \ifnum\@tempdima<\z@\@tempdima=-\@tempdima\fi
      \@tempdimb=#2\relax
      \ifnum\@tempdimb<\z@\@tempdimb=-\@tempdimb\fi
      \advance\@tempdimb\@tempdima
      \ifnum\@tempdimb=\z@
        \@tempdimc=\z@
      \else
        \multiply\@tempdima 8\relax
        \pIIe@divide\@tempdima\@tempdimb\@tempdimc
        \advance\@tempdimc -4pt
        \multiply\@tempdimc 2
        \edef\pIIe@tempa{\strip@pt\@tempdimc}%
        \@tempdima=\pIIe@tempa\@tempdimc
        \advance\@tempdima 64pt
        \divide\@tempdima 2\relax
        \@dashdim=7pt
        \pIIe@@pyth\pIIe@@pyth\pIIe@@pyth
        \edef\pIIe@tempa{\strip@pt\@dashdim}%
        \@tempdimc=\pIIe@tempa\@tempdimb
        \global\divide\@tempdimc 8
      \fi
      \edef\x{\endgroup#3=\the\@tempdimc}%
    \x}
  \newcommand*\pIIe@@pyth{%
    \pIIe@divide\@tempdima\@dashdim\@tempdimc
    \advance\@dashdim\@tempdimc
    \divide\@dashdim\tw@}
  \newcommand*\pIIe@divide[3]{%
    \begingroup
    \dimendef\Numer=254\relax \dimendef\Denom=252\relax
    \countdef\Num=254\relax   \countdef\Den=252\relax
    \countdef\I=250\relax     \countdef\Numb=248\relax
    \Numer #1\relax \Denom #2\relax
    \ifdim\Denom<\z@ \Denom -\Denom \Numer=-\Numer \fi
    \ifdim\Numer<\z@ \def\sign{-}\Numer=-\Numer \else \def\sign{}\fi
    \ifdim\Denom=\z@
      \edef\Q{\strip@pt\maxdimen}%
      \PackageWarning{pict2e}%
        {Division by 0, \sign\strip@pt\maxdimen\space used}{}%
    \else
      \Num=\Numer \Den=\Denom
      \Numb=\Num \divide\Numb\Den
      \ifnum\Numb>16383
        \edef\Q{\strip@pt\maxdimen}%
        \PackageWarning{pict2e}%
          {Division overflow, \sign\strip@pt\maxdimen\space used}{}%
      \else
        \edef\Q{\number\Numb.}%
        \multiply \Numb\Den \advance\Num -\Numb
        \I=6\relax
        \@whilenum \I>\z@ \do{\pIIe@@divide\advance\I\m@ne}%
      \fi
    \fi
    \edef\tempend{\noexpand\endgroup\noexpand#3=\sign\Q\p@}%
    \tempend}
  \def\pIIe@@divide{%
    \@whilenum \Num>214748364 \do{\divide\Num\tw@ \divide\Den\tw@}%
    \multiply \Num 10
    \Numb=\Num \divide\Numb\Den
    \edef\Q{\Q\number\Numb}%
    \multiply \Numb\Den \advance \Num -\Numb
    \ifnum\Num>\z@\else\I=0\fi}
  \newcommand*\pIIe@checkslopeargsline[2]{%
    \pIIe@checkslopeargs{#1}{#2}{16383}}
  \newcommand*\pIIe@checkslopeargsvector[2]{%
    \pIIe@checkslopeargs{#1}{#2}{1000}}
  \newcommand*\pIIe@checkslopeargs[3]{%
    \def\@tempa{#1}\expandafter\pIIe@checkslopearg\@tempa.:{#3}%
    \def\@tempa{#2}\expandafter\pIIe@checkslopearg\@tempa.:{#3}%
    \ifdim #1\p@=\z@ \ifdim #2\p@=\z@ \@badlinearg \fi\fi}
  \def\pIIe@checkslopearg #1.#2:#3{%
    \def\@tempa{#1}%
    \ifx\@tempa\empty\def\@tempa{0}\fi
    \ifx\@tempa\space\def\@tempa{0}\fi
    \ifnum\ifnum\@tempa<\z@-\fi\@tempa>#3\@badlinearg \fi}
  \def\@badlinearg{\PackageError
    {pict2e}{Bad \protect\line\space or \protect\vector\space argument}{}}
  \def\line(#1,#2)#3{%
    \pIIe@checkslopeargsline{#1}{#2}%
    \@tempdima=#1pt\relax \@tempdimb=#2pt\relax
    \@linelen #3\unitlength
    \ifdim\@linelen<\z@ \@badlinearg \else \@sline \fi}
  \def\@sline{%
    \begingroup
    \ifdim\@tempdima=\z@
      \ifdim\@tempdimb<\z@\@linelen-\@linelen\fi
      \@ydim=\@linelen
      \@xdim=\z@
    \else
      \ifdim\@tempdimb=\z@
        \ifdim\@tempdima<\z@\@linelen-\@linelen\fi
        \@xdim=\@linelen
        \@ydim=\z@
      \else
        \ifnum\@tempdima<\z@\@linelen-\@linelen\fi
        \pIIe@divide\@tempdimb\@tempdima\dimen@
        \@ydim=\strip@pt\dimen@\@linelen
        \@xdim=\@linelen
      \fi
    \fi
    \pIIe@moveto\z@\z@
    \pIIe@lineto\@xdim\@ydim
    \pIIe@strokeGraph
    \endgroup}
  \def\vector(#1,#2)#3{%
    \begingroup
    \pIIe@checkslopeargsvector{#1}{#2}%
    \@tempdima=#1pt\relax \@tempdimb=#2pt\relax
    \@linelen#3\unitlength
    \ifdim\@linelen<\z@ \@badlinearg \else
      \pIIe@pyth{\@tempdima}{\@tempdimb}\dimen@
      \ifdim\@tempdima=\z@
      \else\ifdim\@tempdimb=\z@
        \else
          \pIIe@divide\dimen@{\@tempdima}\@xdim
          \@linelen\strip@pt\@xdim\@linelen
          \ifdim\@linelen<\z@\@linelen-\@linelen\fi
        \fi
      \fi
      \pIIe@divide{\@tempdimb}\dimen@\@ydim
      \pIIe@divide{\@tempdima}\dimen@\@xdim
      \pIIe@concat\@xdim\@ydim{-\@ydim}\@xdim\z@\z@
      \pIIe@vector
      \pIIe@fillGraph
    \fi
    \endgroup}
  \newcommand*\pIIe@vector{}
  \newcommand*\pIIe@FAL{}\newcommand*\pIIe@FAW{}\newcommand*\pIIe@CAW{}
  \newcommand*\pIIe@FAI{}
  \newcommand*\pIIe@@firstnum{}\newcommand*\pIIe@@secondnum{}
  \iffalse% the pstricks values gives too small arrows. (RN)
  \AtBeginDocument{%
    \@ifpackageloaded{pstricks}{%
      \def\pIIe@FAL{\psk@arrowlength}%
      \def\pIIe@FAW{\expandafter\pIIe@@secondnum\psk@arrowsize}%
      \def\pIIe@CAW{\expandafter\pIIe@@firstnum\psk@arrowsize}%
      \def\pIIe@FAI{\psk@arrowinset}%
      \def\pIIe@@firstnum#1 #2 {#1\p@}%
      \def\pIIe@@secondnum#1 #2 {#2}%
    }{}%
  }
  \fi
  \newcommand*\pIIe@vector@ltx{%
    \@ydim\pIIe@FAW\@wholewidth \advance\@ydim\pIIe@CAW\relax
    \@ovxx\pIIe@FAL\@ydim
    \@xdim\@linelen \advance\@xdim-\@ovxx
    \divide\@ydim\tw@
    \divide\@ovxx\tw@ \advance\@ovxx\@xdim
    \@ovyy\@ydim
    \divide\@ovyy\tw@ \advance\@ovyy-\pIIe@FAI\@ydim
    \pIIe@bezier@QtoC\@linelen\@ovxx\@ovro
    \pIIe@bezier@QtoC\z@\@ovyy\@ovri
    \pIIe@bezier@QtoC\@xdim\@ovxx\@clnwd
    \pIIe@bezier@QtoC\@ydim\@ovyy\@clnht
    \pIIe@moveto\@linelen\z@
    \pIIe@curveto\@ovro{-\@ovri}\@clnwd{-\@clnht}\@xdim{-\@ydim}%
    \ifdim\@xdim>\z@
      \pIIe@lineto\@xdim{-\@halfwidth}%
      \pIIe@lineto\z@{-\@halfwidth}%
      \pIIe@lineto\z@{\@halfwidth}%
      \pIIe@lineto\@xdim{\@halfwidth}%
    \fi
    \pIIe@lineto\@xdim\@ydim
    \pIIe@curveto\@clnwd\@clnht\@ovro\@ovri\@linelen\z@}
  \newcommand*\pIIe@vector@pst{%
    \@ydim\pIIe@FAW\@wholewidth \advance\@ydim\pIIe@CAW\relax
    \@ovxx\pIIe@FAL\@ydim
    \@xdim\@linelen \advance\@xdim-\@ovxx
    \divide\@ydim\tw@
    \@ovyy\@ydim \advance\@ovyy-\@halfwidth
    \@ovdx\pIIe@FAI\@ovxx
    \pIIe@divide\@ovdx\@ydim\@tempdimc
    \@ovxx\strip@pt\@ovyy\@tempdimc
    \advance\@ovxx\@xdim
    \advance\@ovdx\@xdim
    \pIIe@moveto\@linelen\z@
    \pIIe@lineto\@xdim{-\@ydim}%
    \ifdim\@xdim>\z@
      \pIIe@lineto\@ovxx{-\@halfwidth}%
      \pIIe@lineto\z@{-\@halfwidth}%
      \pIIe@lineto\z@{\@halfwidth}%
      \pIIe@lineto\@ovxx{\@halfwidth}%
    \else
      \pIIe@lineto\@ovdx\z@
    \fi
    \pIIe@lineto\@xdim\@ydim
    \pIIe@lineto\@linelen\z@}
    \def\@circle#1{\begingroup \@tempswafalse\pIIe@circ{#1}}
    \def\@dot#1{\begingroup \@tempswatrue\pIIe@circ{#1}}
  \newcommand*\pIIe@circ[1]{%
      \@tempdima#1\unitlength
      \ifdim\@tempdima<\z@ \pIIe@badcircarg \fi
      \divide\@tempdima\tw@
      \pIIe@circle\@tempdima
      \if@tempswa \pIIe@fillGraph \else \pIIe@strokeGraph \fi
    \endgroup}
  \newcommand*\pIIe@circle[1]{%
    \begingroup
    \buttcap
    \pIIe@qcircle[1]\z@{#1}\pIIe@qcircle  \@ne{#1}%
    \pIIe@qcircle  \tw@{#1}\pIIe@qcircle\thr@@{#1}%
    \endgroup}
  \newcommand*\pIIe@qcircle[3][0]{%
    \begingroup
      \@ovro#3\relax \@ovri0.55228474983\@ovro
      \@tempdimc\@ovri \advance\@tempdimc-\@ovro
      \ifnum#1>\z@ \@tempswatrue \else \@tempswafalse \fi
      \ifcase#2\relax
        \pIIe@@qcircle\@ovro\z@\z@\@ovri\@tempdimc\@ovro{-\@ovro}\@ovro
      \or
        \pIIe@@qcircle\z@\@ovro{-\@ovri}\z@{-\@ovro}\@tempdimc{-\@ovro}{-\@ovro}%
      \or
        \pIIe@@qcircle{-\@ovro}\z@\z@{-\@ovri}{-\@tempdimc}{-\@ovro}\@ovro{-\@ovro}%
      \or
        \pIIe@@qcircle\z@{-\@ovro}\@ovri\z@\@ovro{-\@tempdimc}\@ovro\@ovro
      \fi
    \endgroup}
  \newcommand*\pIIe@@qcircle[8]{%
    \if@tempswa\pIIe@moveto{#1}{#2}\fi \pIIe@rcurveto{#3}{#4}{#5}{#6}{#7}{#8}}
  \newcommand*\pIIe@badcircarg{%
    \PackageError{pict2e}%
      {Illegal argument in \protect\circle(*), \protect\oval, \protect\arc(*) or
      \protect\circlearc.}%
      {The radius of a circle, dot, arc or oval corner must be greater than zero.}}%
  \newcommand*\maxovalrad{20pt}
  \newcommand*\pIIe@defaultUL[2]{%
    \afterassignment\pIIe@def@UL\dimen@#2\unitlength\relax{#1}{#2}}
  \newcommand*\pIIe@def@UL{}
  \def\pIIe@def@UL#1\relax#2#3{%
    \edef#2{\the\dimen@}}
  \newcommand*\pIIe@maxovalrad{}
  \renewcommand*\oval[1][\maxovalrad]{%
    \begingroup \pIIe@defaultUL\pIIe@maxovalrad{#1}%
      \ifdim\pIIe@maxovalrad<\z@ \pIIe@badcircarg \fi
      \pIIe@oldoval}
  \def\@oval(#1,#2)[#3]{%
    \@ovxx#1\unitlength \divide\@ovxx\tw@
    \@ovyy#2\unitlength \divide\@ovyy\tw@
    \@tempdimc \ifdim\@ovyy>\@ovxx \@ovxx \else \@ovyy \fi
    \ifdim\pIIe@maxovalrad<\@tempdimc \@tempdimc\pIIe@maxovalrad\relax \fi
    \@xdim\@ovxx \advance\@xdim-\@tempdimc
    \@ydim\@ovyy \advance\@ydim-\@tempdimc
    \pIIe@get@quadrants{#3}%
    \ifnum15=\@tempcnta \buttcap \fi
    \@tempswatrue
    \ifnum9=\@tempcnta
      \pIIe@qoval\z@{-\@ovyy}{\@xdim}{-\@ovyy}\thr@@\@tempdimc\@ovxx\z@
      \@tempcnta\@ne
    \fi
    \pIIe@qoval\@ovxx\z@\@ovxx\@ydim\z@\@tempdimc\z@\@ovyy
    \pIIe@qoval\z@\@ovyy{-\@xdim}\@ovyy\@ne\@tempdimc{-\@ovxx}\z@
    \pIIe@qoval{-\@ovxx}\z@{-\@ovxx}{-\@ydim}\tw@\@tempdimc\z@{-\@ovyy}%
    \pIIe@qoval\z@{-\@ovyy}{\@xdim}{-\@ovyy}\thr@@\@tempdimc\@ovxx\z@
    \pIIe@strokeGraph
    \endgroup}
  \newcommand*\pIIe@qoval[8]{%
    \ifodd\@tempcnta
      \if@tempswa\pIIe@moveto{#1}{#2}\fi
      \pIIe@lineto{#3}{#4}\pIIe@qcircle{#5}{#6}\pIIe@lineto{#7}{#8}%
      \@tempswafalse
    \else
      \@tempswatrue
    \fi
    \divide\@tempcnta\tw@}
  \newcommand*\pIIe@get@quadrants[1]{%
    \@ovttrue \@ovbtrue \@ovltrue \@ovrtrue \@tempcnta\z@
    \@tfor\reserved@a:=#1\do{\csname @ov\reserved@a false\endcsname}%
    \if@ovr \if@ovb\@setfpsbit2\fi \if@ovt\@setfpsbit4\fi \fi
    \if@ovl \if@ovb\@setfpsbit1\fi \if@ovt\@setfpsbit8\fi \fi}
  \def\@bezier#1(#2,#3)(#4,#5)(#6,#7){%
    \ifnum #1=\z@
      \@killglue
      \begingroup
      \@ovxx#2\unitlength \@ovyy#3\unitlength
      \@ovdx#4\unitlength \@ovdy#5\unitlength
      \@xdim#6\unitlength \@ydim#7\unitlength
      \pIIe@bezier@QtoC\@ovxx\@ovdx\@ovro
      \pIIe@bezier@QtoC\@ovyy\@ovdy\@ovri
      \pIIe@bezier@QtoC\@xdim\@ovdx\@clnwd
      \pIIe@bezier@QtoC\@ydim\@ovdy\@clnht
      \pIIe@moveto\@ovxx\@ovyy
      \pIIe@curveto\@ovro\@ovri\@clnwd\@clnht\@xdim\@ydim
      \pIIe@strokeGraph
      \endgroup
      \ignorespaces
    \else
      \pIIe@old@bezier{#1}(#2,#3)(#4,#5)(#6,#7)
    \fi}
    \newcommand*\pIIe@bezier@QtoC[3]{%
      \@tempdimc#1\relax      \advance\@tempdimc-#2\relax
      \divide\@tempdimc\thr@@ \advance\@tempdimc #2\relax
      #3\@tempdimc}
  \ifx\undefined\@arclen \newdimen\@arclen \fi
  \ifx\undefined\@arcrad \newdimen\@arcrad \fi
  \ifx\undefined\@tempdimd \newdimen\@tempdimd \fi
  \newcommand*\pIIe@arc[6][0]{%
    \@arcrad #4\relax
    \ifdim \@arcrad<\z@ \pIIe@badcircarg \else
      \@arclen #6\p@ \advance\@arclen -#5\p@
      \ifdim \@arclen<\z@ \def\sign{-}\else\def\sign{}\fi
      \ifdim \sign\@arclen>720\p@
        \PackageWarning {pict2e}{The arc angle is reduced to -720..720}%
        \@whiledim \sign\@arclen>720\p@ \do {\advance\@arclen-\sign360\p@}%
        \@tempdima #5\p@ \advance\@tempdima \@arclen
        \edef\@angleend{\strip@pt\@tempdima}%
        \pIIe@@arc{#1}{#2}{#3}{#4}{#5}{\@angleend}%
      \else
        \pIIe@@arc{#1}{#2}{#3}{#4}{#5}{#6}%
      \fi
    \fi}
  \newcommand*\pIIe@@arc[6]{%
    \begingroup
    \ifdim \sign\@arclen>90\p@
      \divide\@arclen 2
      \@tempdima #5\p@ \advance\@tempdima \@arclen
      \edef\@anglemid{\strip@pt\@tempdima}%
      \def\@temp{\pIIe@@arc{#1}{#2}{#3}{#4}{#5}}%
      \expandafter\@temp\expandafter{\@anglemid}%
      \def\@temp{\pIIe@@arc{2}{#2}{#3}{#4}}%
      \expandafter\@temp\expandafter{\@anglemid}{#6}%
    \else
      \CalculateSin{#5}\CalculateCos{#5}%
      \@tempdima\UseCos{#5}\@arcrad \advance\@tempdima #2\relax
      \@tempdimb\UseSin{#5}\@arcrad \advance\@tempdimb #3\relax
      \ifcase #1\relax
          \pIIe@lineto\@tempdima\@tempdimb
      \or \pIIe@moveto\@tempdima\@tempdimb
      \or
      \else \PackageWarning {pict2e}%
            {Illegal obligatory argument in \protect\circlearc.}%
      \fi
      \@tempdimc\@arclen \divide\@tempdimc\@iv
      \edef\@angle{\strip@pt\@tempdimc}\CalculateTan{\@angle}%
      \@linelen\UseTan{\@angle}\@arcrad \@linelen4\@linelen \divide\@linelen\thr@@
      \advance\@tempdima-\UseSin{#5}\@linelen
      \advance\@tempdimb \UseCos{#5}\@linelen
      \pIIe@add@nums\@tempdima\@tempdimb
      \CalculateSin{#6}\CalculateCos{#6}%
      \@tempdima \UseCos{#6}\@arcrad \advance\@tempdima #2\relax
      \@tempdimb \UseSin{#6}\@arcrad \advance\@tempdimb #3\relax
      \@tempdimc \UseSin{#6}\@linelen \advance\@tempdimc \@tempdima
      \@tempdimd-\UseCos{#6}\@linelen \advance\@tempdimd \@tempdimb
      \pIIe@add@nums\@tempdimc\@tempdimd
      \pIIe@add@CP\@tempdima\@tempdimb
      \pIIe@addtoGraph\pIIe@curveto@op
    \fi
    \endgroup}
  \newcommand*\arc{\@ifstar{\@tempswatrue\@arc}{\@tempswafalse\@arc}}
  \newcommand*\@arc[2][0,360]{\@@arc(#1){#2}}
  \def\@@arc(#1,#2)#3{%
    \if@tempswa
      \pIIe@moveto\z@\z@
      \pIIe@arc{\z@}{\z@}{#3\unitlength}{#1}{#2}%
      \pIIe@closepath\pIIe@fillGraph
    \else
      \pIIe@arc[1]{\z@}{\z@}{#3\unitlength}{#1}{#2}%
      \pIIe@strokeGraph
    \fi}
  \let\lp@r( \let\rp@r)
  \def\Line(#1,#2)(#3,#4){\polyline(#1,#2)(#3,#4)}
  \def\polyline(#1,#2){%
    \@killglue
    \pIIe@moveto{#1\unitlength}{#2\unitlength}%
    \@ifnextchar\lp@r{\@polyline}{\PackageWarning{pict2e}%
      {Polygonal lines require at least two vertices!}%
    \ignorespaces}}
  \def\@polyline(#1,#2){%
    \pIIe@lineto{#1\unitlength}{#2\unitlength}%
    \@ifnextchar\lp@r{\@polyline}{\pIIe@strokeGraph\ignorespaces}}
  \def\polygon{%
    \@killglue
    \@ifstar{\begingroup\@tempswatrue\@polygon}%
      {\begingroup\@tempswafalse\@polygon}}
  \def\@polygon(#1,#2){%
    \pIIe@moveto{#1\unitlength}{#2\unitlength}%
    \@ifnextchar\lp@r{\@@polygon}{\PackageWarning{pict2e}%
      {Polygons require at least two vertices!}%
    \ignorespaces}}
  \def\@@polygon(#1,#2){\pIIe@lineto{#1\unitlength}{#2\unitlength}%
    \@ifnextchar\lp@r{\@@polygon}{\pIIe@closepath
      \if@tempswa\pIIe@fillGraph\else\pIIe@strokeGraph\fi
      \endgroup
      \ignorespaces}}
  \def\moveto(#1,#2){%
    \@killglue
    \pIIe@moveto{#1\unitlength}{#2\unitlength}%
    \ignorespaces}
  \def\lineto(#1,#2){%
    \@killglue
    \pIIe@lineto{#1\unitlength}{#2\unitlength}%
    \ignorespaces}
  \def\curveto(#1,#2)(#3,#4)(#5,#6){%
    \@killglue
    \pIIe@curveto{#1\unitlength}{#2\unitlength}{#3\unitlength}{#4\unitlength}%
      {#5\unitlength}{#6\unitlength}%
    \ignorespaces}
  \newcommand*\circlearc[6][0]{%
    \@killglue
    \pIIe@arc[#1]{#2\unitlength}{#3\unitlength}{#4\unitlength}{#5}{#6}%
    \ignorespaces}
  \def\closepath{\pIIe@closepath}
  \def\strokepath{\pIIe@strokeGraph}
  \def\fillpath{\pIIe@fillGraph}
  \ifcase\pIIe@mode\relax
  \or
    \def\buttcap{\special{ps:: 0 setlinecap}}
    \def\roundcap{\special{ps:: 1 setlinecap}}
    \def\squarecap{\special{ps:: 2 setlinecap}}
    \def\miterjoin{\special{ps:: 0 setlinejoin}}
    \def\roundjoin{\special{ps:: 1 setlinejoin}}
    \def\beveljoin{\special{ps:: 2 setlinejoin}}
  \or
    \def\buttcap{\pdfliteral{0 J}}
    \def\roundcap{\pdfliteral{1 J}}
    \def\squarecap{\pdfliteral{2 J}}
    \def\miterjoin{\pdfliteral{0 j}}
    \def\roundjoin{\pdfliteral{1 j}}
    \def\beveljoin{\pdfliteral{2 j}}
  \fi
  \AtBeginDocument{\@ifundefined{cbezier}{\newcommand}{\renewcommand}*%
      \cbezier[2][0]{\pIIe@@cbezier[#1]#2}%
    \@ifdefinable\pIIe@@cbezier{}%
    \def\pIIe@@cbezier#1)#2(#3)#4(#5)#6({\@cbezier#1)(#3)(#5)(}%
    \def\@cbezier[#1](#2,#3)(#4,#5)(#6,#7)(#8,#9){%
      \@killglue
      \pIIe@moveto{#2\unitlength}{#3\unitlength}%
      \pIIe@curveto{#4\unitlength}{#5\unitlength}%
        {#6\unitlength}{#7\unitlength}{#8\unitlength}{#9\unitlength}%
      \pIIe@strokeGraph
      \ignorespaces}%
  }
\else
  \renewcommand*\oval[1][]{\pIIe@oldoval}
  \newcommand*\maxovalrad{20pt}
  \newcommand*\OriginalPictureCmds{}
\fi
\Gin@codes
\let\Gin@codes\relax
\endinput
%%
%% End of file `pict2e.sty'.

